Omni-SMoLA: Boosting Generalist Multimodal Models with Soft Mixture of Low-rank Experts

Large multi-modal models (LMMs) exhibit remarkable performance across numerous tasks. However, generalist LMMs often suffer from performance degradation when tuned over a large collection of tasks. Recent research suggests that Mixture of Experts (MoE) architectures are useful for instruction tuning, but for LMMs of parameter size around O(50-100B), the prohibitive cost of replicating and storing the expert models severely limits the number of experts we can use. We propose Omni-SMoLA, an architecture that uses the Soft MoE approach to (softly) mix many multimodal low rank experts, and avoids introducing a significant number of new parameters compared to conventional MoE models. The core intuition here is that the large model provides a foundational backbone, while different lightweight experts residually learn specialized knowledge, either per-modality or multimodally. Extensive experiments demonstrate that the SMoLA approach helps improve the generalist performance across a broad range of generative vision-and-language tasks, achieving new SoTA generalist performance that often matches or outperforms single specialized LMM baselines, as well as new SoTA specialist performance.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

\mc{P1: background and history.}

Problem: LMMs on downstream multitasks.

Currently specialized model is the mainstream solution. However, each task need a specialized model. when the volume of downstream tasks increase, the number of downstream specialized models and the computational cost also increase tremendously.
We propose a solution to only tune a small number of parameters and make the generalist LMM performance good on multiple downstream tasks. 


\noindent\mc{P2: discuss the challenges of multimodal multitask.}
The main challenges of tuning LMMs for downstream multitasks include:
\begin{itemize}
    \item Multi-task: build a single model to solve multi-task is challenging, especially dense model. Intuitively, this strongly rely on the learnability of the model to force to distinguiash between tasks. Previous empirical study shows the performance is not very good, especially when the number of tasks increases, the performance drops obviously \todo{citation needed}.
    \item Multimodal: the complexity of the problem increases in the nature of multimodal tasks. In a mixture of multiple multimodal tasks, there are some tasks strongly rely on visual features while others might reply on text features. 
    \item Scale of parameters: the increasing of volume of parameters of models. 
\end{itemize}


\noindent\mc{P3: we propose M3LoRA which can handle above 3 challenges}
We propose the Mix of Multi-modal LoRA~(M$^3$LoRA). \mc{Add brief description.}

How our approch handle above 3 challenges:
\begin{itemize}
    \item M$^3$: (multimodal) the capability to dynamically learn visual experts, text experts and common experts for different multimodal tasks. (multitask) MoE mechanism make the model a good fit for multitasks simultaneously.
    \item Our proposed two step solution make sure the M$^3$LoRA start from a high quality initial $\theta^*$. 
    \item LoRA.
\end{itemize}


\noindent\mc{P4: contribution summary}
To summary, the main contributions of this work includes:
\begin{itemize}
    \item We propose M$^3$LoRA - mixture of multi-model LoRA experts. 
    \item We propose a comprehensive multimodal multitask solution. 
    \item Our approach shows incredible results. 
\end{itemize}


==> sec/3_approach.tex <==
\section{Methodology}
\subsection{Mixture-of-Experts}

% The objective of sparsely-activated model design is to support conditional computation and increase the parameter count of neural models like Transformers while keeping the floating point operations (FLOPs) for each input example constant. Mixture-of-Experts (MoE) Transformer models~\citep{shazeer2017outrageously, fedus2021switch,lepikhin2020gshard,zuo2021taming} achieve this by using $N$ feed-forward networks (FFN), namely ``experts" denoted as $\mathbb{E}_{i=1}^N$, each with its own set of learnable weights that compute different representations of an input token $x$ based on context. In order to sparsify the network to keep the FLOPs constant, there is an additional gating network $\mathbb{G}$ whose output is a sparse $N$-dimensional vector to route each token via a few of these experts. Note that, a sparse model with $N=1$ corresponding to only one FFN layer in each Transformer block collapses to the traditional dense model. 

% Consider $x_s$ as the input token representation in the $s^{th}$ position to the MOE layer comprising of the $\{\mathbb{E}\}_{i=1}^N$ expert FFNs. Also, consider $w^{in}_i$ and $w^{out}_i$ to be the input and output projection matrices for $i^{th}$ expert. Expert output  $\mathbb{E}_i(x_s)$ is given by:

The design philosophy behind sparse activation models is centered around enhancing conditional computation capabilities and scale parameters in neural architectures such as Transformers, all while maintaining floating point operations (FLOPs) as constant per input instance. The Mixture-of-Experts (MoE) Transformer models~\cite{shazeer2017outrageously, fedus2021switch,lepikhin2020gshard,zuo2021taming}, stand out in this regard, employing $N$ feed-forward networks (FFN), referred to as “experts,” symbolized as $\mathbb{E}_{i=1}^N$. Each of these experts boasts its unique set of trainable weights, enabling them to craft distinct representations of an input token $x$ contingent on the contextual information.

To realize network sparsity and thereby keep the FLOPs in check, the architecture incorporates an additional gating network $\mathbb{G}$ . This network outputs a sparse $N$-dimensional vector, serving the purpose of directing each token to a select number of experts. Note that when the model is configured to $N=1$, indicating the presence of a single FFN layer in each Transformer block, it effectively reverts to a conventional dense model.

Focusing on a specific instance, we denote $x_s$ as the representation of the input token situated at the $s^{th}$ position within the MoE layer, which encompasses the set of expert FFNs  $\{\mathbb{E}\}_{i=1}^N$. Additionally, let \(w^{in}_i\) and \(w^{out}_i\) represent the input and output projection matrices for the $i^{th}$ expert, respectively. Under these considerations, the output $\mathbb{E}_i(x_s)$ generated by expert \(\mathbb{E}_i\) for input token $x_s$ can be expressed as follows:


\begin{equation}
    \mathbb{E}_i(x_s) = w^{out}_i \cdot \text{GeLU} (w^{in}_i \cdot x_s)
\end{equation}

\noindent Consider $\mathbb{G}(x_s)$ to be output of the gating network. Output of the sparse MoE layer is given by:

\begin{equation}
\label{eq:moe}
    h(x_s)=\sum_i \mathbb{G}(x_s)_i\ \mathbb{E}_i(x_s) 
\end{equation}

\noindent where $\mathbb{G}(x_s)_i$ the $i^{th}$ logit of the output of $\mathbb{G}(x_s)$ denotes the probability of selecting expert $\mathbb{E}_i$. 


In order to keep the number of FLOPs in the sparse Transformer to be the same as that of a dense one, the gating mechanism can be constrained to route each token to only one expert FFN, i.e. $\sum_i \mathbb{G}_t(x_s)_i = 1$.

\subsection{Low-rank Adaptation (LoRA)}

Low-Rank Adaptation (LoRA)~\cite{hu2021lora} is a technique designed to enhance the adaptability of pretrained Transformer models to new tasks with a minimal increase in the number of trainable parameters. This method specifically targets the attention mechanism, aiming to fine-tune the attention weights in an efficient manner.

Let's denote \( \mathbb{A}_i \) as the attention matrix for the \( i^{th} \) layer of a Transformer model. LoRA introduces two low-rank matrices \( \mathbb{L}_i^{in} \) and \( \mathbb{L}_i^{out} \) for each layer, where \( \mathbb{L}_i^{in} \) is applied to the input of the attention layer, and \( \mathbb{L}_i^{out} \) is applied to the output. The adaptation of the attention weights can be represented as:

\begin{equation}
\mathbb{A}_i'= \mathbb{A}_i + \mathbb{L}_i^{in} \mathbb{L}_i^{out}
\end{equation}

where \( \mathbb{A}_i' \) represents the adapted attention weights for the \( i^{th} \) layer, and \( T \) denotes the transpose operation. The rank of \( \mathbb{L}_i^{in} \) and \( \mathbb{L}_i^{out} \) is typically much smaller than the dimension of \( \mathbb{A}_i \), resulting in a compact and efficient adaptation of the attention mechanism.

\subsection{Mixture-of-LoRAs}

\subsection{Soft Merging Mechanism}


\begin{figure*}[htb!]
  
 		\centering
	\includegraphics[width=0.8\linewidth]{./figs/mlora_new.pdf}
 	  	\caption{M$^4$LoRA model architecture. The M$^4$LoRA is built on linear layers for maximum flexibility.  }
 	 	 	\label{fig:framework}
 
\end{figure*}


\subsection{Scaling with Low-rank Experts}

\noindent\textbf{Parameter Efficiency and Memory Reduction.} The integration of LoRA into the MoE framework results in a substantial reduction in the number of parameters required for adaptation compared to traditional MoE. The low-rank matrices introduced by LoRA are of significantly lower dimensionality than the full-rank feedforward layers, ensuring that the parameter increase is minimal. Not only does this lead to a leaner model, but it also reduces memory requirements, making it feasible to increase the number of experts to enhance performance.

\noindent\textbf{Alternative Scaling Dimensions.}
Traditional scaling methods in neural networks often involve increasing the size of the model, either by adding more layers or increasing the dimensionality of the existing layers. The proposed method, on the other hand, introduces an alternative scaling dimension. By leveraging sparse activation and parameter-efficient adaptation, the proposed method achieves scaling through increased low-rank expert numbers, rather than sheer size.

\noindent \textbf{Extensibility for Future Growth.} The design of the proposed method inherently supports extensibility, accommodating future growth and adaptations with ease. As the requirements of a task evolve, additional LoRA modules can be seamlessly integrated into the architecture, enhancing the model’s capability without necessitating a complete overhaul. This stands in stark contrast to traditional scaling methods, which often require predefined dimensions and layer numbers, limiting the model’s size to adapt to changing scenarios.

==> sec/5_discussion.tex <==
\section{Discussion}
%temporarily - for collect additional thinkings and explana-409tions, can remove]

\subsection{Multitask learning.}

Most multitask learning approaches aim to find one single model to perform well on all tasks~\cite{zhang2021survey,lin2019pareto}. 
The challenge of multitask learning is, there are some tasks which conflict with each other, and no single model can optimize the performance on all tasks simultaneously~\cite{zhang2021survey,lin2019pareto}. 

When fine-tuning a LMM on multiple downstream tasks, the common approach is to build a mixture of these multiple tasks and run the tuning. This approach lines in the linear weighted scalarization category of multitask learning~\cite{zhang2021survey,lin2019pareto,caruana1997multitask}:

Given a list of $m$ tasks ${t_1, t_2, ..., t_m}$, the MTL loss is: 
\begin{equation}
    min_\theta\ \mathcal{L}(\theta) = (\mathcal{L}_1(\theta), \mathcal{L}_2(\theta), ..., \mathcal{L}_m(\theta))^T
\end{equation}
where $\mathcal{L}_i$ is the text generation loss~\cite{pmlr-v139-cho21a} of task $t_i$, written as
\begin{equation}
    \mathcal{L}_i = - \sum_{x_i,y_i \in t_i} \log P_{\theta}(y_i | x_i)
\end{equation}

When fine-tuning on a mixture of multiple downstream tasks at the same time, the unified loss that optimizes the LMM on all tasks can be written as:
\begin{equation} 
\begin{split}
    \mathcal{L} &= - \sum_{(x,y) \in D} log P_\theta (y|x) \\ 
    &= - \sum_{(x,y) \in t_1} log P_\theta (y|x) - ... - \sum_{(x,y) \ in t_m}  log P_\theta (y|x) \\
    &= \sum_{i=1}^m \mathcal{L}_i
\end{split}
\end{equation}
This corresponds to the linear weighted scalarization approach for multitask learning, with task specific weight equals to 1. 

A lot of previous multitask learning works shows that this unified loss is unable to find the optimal solution for all tasks, but can only find a trade-off solution (our $\theta^*$), especially when some tasks conflict with each other~\cite{lin2019pareto} . 
However, this trade-off solution is always far behind task specific optimal which fine-tunes specifically on a single task[need ref here]. 

\paragraph{MoE.} 
% common sense, a lot of references if needed
MoE decompose the multitask problem to several sub-problems. In other words, MoE separates the parameter space and activate a separate sub-model to correspond to every task.

Thus the goal becomes to optimize:
\begin{equation}
    P_{x \in t_i}(\theta_i | x) P_{\theta_i} (y | x)
\end{equation}
MoE, especially benefitting from its sparsity feature, seperates the parameter space to activate different experts for different tasks.
In this case, it breaks the problem of single model for multitasks into different models for different, separate tasks, though these models share most of the parameters.
Thus, the conflicting tasks issue can be resolved by activating different experts, and MoE achieves close to or even better than specilized model's performance.


\subsection{Why $\theta^*$ is important?}
The first step of our M$^4$LoRA solution is to find a good trade-off solution $\theta^*$. Our experiments demonstrate the effectiveness of $\theta^*$ from empirical perspective. Below we provide 3 interpretation to discuss the importance of $\theta^*$ from theoretical perspective. 

\paragraph{Initialization.}


\paragraph{Hypothesis space search.}
- LoRA as well as M$4$LoRA correspond to a relatively small hypo space
to make it easier to go to $\theta^*_i$ from every where, we design it to go to $\theta^*$ at first.

- also more stable and not fully rely on optimization.

\paragraph{Learn common representation.}


\subsection{Time Complexity Analysis}

Given $X \in R^{N \times d_1}$ and $Y \in R^{N \times d_2}$, $E$ is the number of experts and $r$ is the rank of per expert. 
The dispatcher $D$ and combiner $C$ both in $R^{E \times N}$ corresponding to $E$ experts. The parameters to compute $D, C$, denoted by $\Phi \in R^{E \times d_1}$. 
Each expert has two parameter weight matrices $W_i^{in} \in R^{r \times d_1}$, $W_i^{out} \in R^{d_2 \times r}$. 

To compute $D$ and $C$ takes $O(E \times d_1 \times N)$. 

To compute the dispatched input $(DX) \in R^{E \times d_1}$ takes $O(E \times N \times d_1).

Then for $i$-th expert's corresponding dispatched input $(DX)_{i,:} \in R^{1 \times d_1}$, to compute Eq~\ref{eq:expert_lora} to obtain $\tilde{y}_i \in R^{d_2 \times 1}$ takes $O(r\times d_1 + r\times d_2)$. 
To compute output $\tilde{y}_i$ for all $E$ experts in total takes $O(rd_1E + rd_2E)$.

Then for Eq~\ref{eq:final}, the total increased computational cost by adding \sysname is $O(N \times E \times d_2 + N\times d_2)$.

So in total it takes $O(ENd_1 + ENd_1 + Erd_1 + Erd_2 + ENd_2 + Nd_2)$. 
Let $d_{max} = \max\{d_1, d_2\}$, the time complexity is written as $O(ENd_{max})$. 

So for one layer, it increases the time complexity from $O(Nd_1 d_2)$~(compute the original $XW^*$) to $O(Nd_1d_2 + ENd_{max})$. Since he number of expert $E$ is always $\ll \min \{d_1, d_2\}$, the increased time complexity can be ignored. 


